Logical Entity Representation in Knowledge-Graphs for Differentiable Rule Learning

Probabilistic logical rule learning has shown great strength in logical rule mining and knowledge graph completion. It learns logical rules to predict missing edges by reasoning on existing edges in the knowledge graph. However, previous efforts have largely been limited to only modeling chain-like Horn clauses such as $R_1(x,z)\land R_2(z,y)\Rightarrow H(x,y)$. This formulation overlooks additional contextual information from neighboring sub-graphs of entity variables $x$, $y$ and $z$. Intuitively, there is a large gap here, as local sub-graphs have been found to provide important information for knowledge graph completion. Inspired by these observations, we propose Logical Entity RePresentation (LERP) to encode contextual information of entities in the knowledge graph. A LERP is designed as a vector of probabilistic logical functions on the entity's neighboring sub-graph. It is an interpretable representation while allowing for differentiable optimization. We can then incorporate LERP into probabilistic logical rule learning to learn more expressive rules. Empirical results demonstrate that with LERP, our model outperforms other rule learning methods in knowledge graph completion and is comparable or even superior to state-of-the-art black-box methods. Moreover, we find that our model can discover a more expressive family of logical rules. LERP can also be further combined with embedding learning methods like TransE to make it more interpretable.

==> body/20_problem.tex <==
\label{sec:formulation}

\paragraph{Chain-like Horn Clauses} are a set of first-order logic rules that have been widely studied in logical rule learning \citep{sadeghian2019drum,yang2017differentiable}. Formally, the task setting provides a knowledge graph $G=\{(s,r,o)|s,o\in\mathcal{E},r\in\mathcal{R}\}$, where $\mathcal{E}$ is the set of entities and $\mathcal{R}$ is the set of relation types. The chain-like Horn clauses are defined as in Equation ~\ref{eq:chain_rule}, where $x, y, z_k\in \mathcal{E}$ (for $k\in[1, K-1]$) and $H, r_k \in \mathcal{R}$ (for $k\in[1, K]$). The ``reverse'' edges $r'(z,z')=r(z',z)$ are often added to the edge type set $\gR$. $r_1(x,z_1) \land \cdots \land r_K(z_{K-1},y)$ is typically named the ``body'' of the rule.

A computational convenience of this formulation is that, if $x$ is known, the rule can be evaluated by computing a sequence of matrix multiplications.
% \heng{\sout{this sentence "the calculation of the clause body if can be computed by matrix multiplications." is not grammatically correct. fix it}}
We can first order entities in $\gE$ from 1 to $n=|\gE|$, let $\rvv_x$ be an $n$-dimensional one-hot vector of $x$'s index, and let $\mA_{r_k}$ be the adjacency matrix of $r_k$. In this way, we can compute $\rvv_x^\top \prod_{k=1}^K \mA_{r_k}$ in $O(Kn^2)$ time, by multiplying from $\mathbf{v}_x^\top$ side in a left-to-right order. It is easy to verify that this result is an $n$-dimensional vector counting how many paths connect $x$ and $y$ following the relation sequence $r_1, r_2\cdots r_K$. This formulation has been widely adopted by previous methods.
% When restricted to the Boolean domain, this corresponds to the vector of $\exists \{z_k\}: \textit{the body is true for } x, y$ on $y$.
% In practice, the result in real domain is often adopted for computation convenience.
% The space efficiency is also beneficial as knowledge graphs can mount up to hundred of thousands of entities.

\paragraph{Logical Entity Representation (\model{})}

In this work, we introduce \model{} in logical rules to provide additional local contextual information for entities in the knowledge graph. A \model{} for entity $e$ is formatted as a vector $\mL(e)=(L_1(e), \cdots, L_m(e))$ where the dimension $m$ is a hyper-parameter. Each $L_i(e)$ is a logical function over $e$'s surrounding sub-graph. To enable efficient evaluation of $L_i(e)$, we limit $L_i(e)$ to a family of \textit{tree-like logical functions} as defined below:

\begin{definition}
\label{def:tree_function}
(Tree-like logical function)

Given a binary predicate set $\gR$, the family of tree-like logical functions $\gT$ is recursively constructed with the following operations:
% Given two entities $x,y$ and the head link to predict $H(x,y)$, a tree-like Horn clause $\mT$ is any rule that can be constructed in the following recursive manner (all $z,z'$, unless otherwise explained, are free variables taking value from $\gE$):

\begin{enumerate}
    \item (True function) $f(w_0) = true$ belongs to $\gT$.
    \item (Chaining) For any $f(w_i)\in\gT$ and $r\in\gR$, $f'(w_{i+1})=\exists w_i: f(w_i)\land r(w_i, w_{i+1})$ also belongs to $\gT$.
    \item (Negation) For any $f(w_i)\in\gT$, $f'(w_i)=\lnot f(w_i)$ belongs to $\gT$.
    \item (Merging) For any $f(w_i),f'(w_{i'})\in\gT$, let $i''=\max(i,i')+1$, after applying substitution $\{w_i\mapsto w_{i''}\}$ and $\{w_{i'}\mapsto w_{i''}\}$ to two functions respectively, $f''(w_{i''})=f(w_{i''})\land f'(w_{i''})$ ($\land$-merging) and $f''(w_{i''})=f(w_{i''})\lor f'(w_{i''})$ ($\lor$-merging) belong to $\gT$.
\end{enumerate}

% then the logical rule $\mB \Rightarrow H(x,y)$ is defined as a tree-like Horn clause $\mT$, where $\mB$ and $H(x,y)$ are the body and head of $\mT$, respectively. We also denote $|\mT|=|\mB|$, $G_\mT$ as the tree composed of variables and edges in $\mB$, and denote $\mB_f=\exists z_1, z_2 \cdots z_{|\mB|-1} \mB$ which quantifies all free variables in $\mB$.

\end{definition}

This definition includes arbitrarily complex functions, but in practice we limit a maximum number of operations. Intuitively, one can think of a function $f(w_i)\in\gT$ as mimicking the shape of a local tree spanning from $w_i$ as in Figure~\ref{fig:framework}(a). Specifically, this is because it gathers information together recursively through logical operations. $\mL(e)$ then serves as a logical contextual representation for $e$'s local surrounding sub-graph. We then extend Equation~\ref{eq:chain_rule} into the following formula to incorporate contextual information from $\mL(e)$:
% Our model extends the original chain-like Horn clauses by extending Equation~\ref{eq:chain_rule} to the following form:
\begin{equation}
    r_1(x,z_1) \land r_2(z_1,z_2) \land \cdots \land r_K(z_{K-1},y)
    \land 
    \left(\bigwedge_{z'\in\{x,y,z_1,\cdots\}}L_{i_{z'}}(z')\right)
    \Rightarrow H(x,y),
    \label{eq:extended_rule}
\end{equation}
where $i_{z'}\in[1..m]$ is an index to select logical functions from \model{}. Now the rule in Figure~\ref{fig:branch}(c) is an example of this form
% $\textit{is\_son\_of}(x,z_1)\land \textit{is\_spouse\_of}(z_1,y) \land L_{i_x}(x)\land L_{i_y}(y) \land L_{i_{z_1}}(z_1) \Rightarrow \textit{is\_mothder\_of}(x,y)$ 
by setting $L_{i_x}(x) = true$, $L_{i_y}(y) = true$, $L_{i_{z_1}}(z_1) = \exists z_2: \textit{is\_son\_of}(z_1,z_2)$.
In fact, this extension does not break the computational efficiency of chain-like Horn clauses (proofs are included in Appendix):


\begin{theorem}
For any rule expressed in Equation~\ref{eq:extended_rule}, if $x$ is known, the evaluation of its LHS over $x$ and all $y\in\gE$ (considering all possible $z_i$), can be determined in $O(Cn^2)$ time where $n=|\gE|$ is the size of the entity set and $C$ is a constant related to the rule.

\label{thm:efficiency}
\end{theorem}

% In the case of knowledge graph completion, $x$ and $H$ is often assumed to be given and models are required to predict $y$. In that case, we also have the following property similar to chain-like rules:
% \begin{corollary}
% For any rule expressed in Equation~\ref{eq:extended_rule}, if $x$ is known, the value of its LHS between $x$ and all $y\in\gE$ considering all possible $z_i$ can be determined in $O(Cn^2)$ time and $O(C'n)$ space where $C'$ is maximum number of .
% \end{corollary}

==> body/40_analysis.tex <==
\label{sec:analysis}

This work is motivated by the hypothesis that contextual information for entities can help logical rules to improve knowledge graph completion. As a verification, we conducted a set of smaller-scale experiments, where we design a simplest extension to existing logical rules. To be specific, within the Equation~\ref{eq:chain_rule}, we add a series of simple logical predicate $\exists z_k': r_k'(z_k', z_k)$ for some of the intermediate entity indices $S'\subset [1..K-1]$. This can be understood as filtering some $z_k$ by the existence of a locally connected edge $r_k'$. This converts Equation~\ref{eq:chain_rule} to the following form:

\begin{equation}
    r_1(x,z_1) \land \cdots \land r_K(z_{K-1},y) \land \left(\bigwedge_{k\in S'} \exists z_k': r_k'(z_k', z_k)\right) \Rightarrow H(x,y)
    \label{eq:simple_extension}
\end{equation}

For this study, we choose to augment  DRUM~\citep{sadeghian2019drum}, a state-of-the-art probabilistic logical rule mining baseline based on Equation~\ref{eq:chain_rule}. The implementation of this extension is very simple. Regardless of the technical designs of the DRUM model, we only included a new family of edges $\gR'=\{r''(u,v)=r(u,v)\land\exists v': r'(v', v), r, r' \in \gR\}$, and replace $\gR$ with $\gR_{aug}=\gR\cup\gR'$. Finally we apply the original DRUM model to $\gR_{aug}$, which is equivalent to modeling Equation~\ref{eq:simple_extension}. We conduct experiments on two common graph completion datasets: Family and Kinship~\citep{kok2007statistical}. Both these datasets consist of kinship graphs, and the task is to complete missing edges between people. As shown in Figure~\ref{fig:motivating_study}, we observe a uniform improvement in DRUM's performance on both datasets when augmented with our rule extensions.

==> body/50_approach.tex <==
\label{sec:framework}

\subsection{Derivation of \model{}}

This section describes our computational modeling of \model{} and how to incorporate it in probabilistic logic rule learning. In Definition~\ref{def:tree_function} we have defined a family of tree-like logical functions which enables efficient evaluation. However, the selection of predicates and its logical form is still discrete and can lead to huge searching complexity. Borrowing ideas from \cite{yang2017differentiable,sadeghian2019drum} we relax \model{} to the probabilistic domain to make its results continuous, which also allows us to use gradient-based methods for optimization.

Figure~\ref{fig:framework}(b) provides an illustration of our method. We compute the tree-like probabilistic logical functions $L^\Theta_i$ parameterized by $\Theta$ by adopting a feed-forward paradigm, and compute intermediate functions $f^\Theta_{j,i}(z_{j,i})$ column by column. The first column contains only $true$ functions $f^\Theta_{0,i}(z_{0,i})=true$. For $j>0$, each $f^\Theta_{j,i}(z_{j,i})$ is constructed from the previous column by 6 possible operations: \textit{true function}, \textit{chaining}, \textit{negation}, \textit{$\land$-merging}, and \textit{$\lor$-merging} from Definition~\ref{def:tree_function}, as well as an additional \textit{copy} operation that simply copies $f^\Theta_{j-1,i}(z_{j-1,i})$. Note that the result of $f^\Theta_{j,i}(z_{j,i})$ over $\gE$ can be represented as a $|\gE|$-dimensional vector $\rvv_{j,i}$. Taking this notation, the formulae for the 6 possible types of $f^\Theta_{j,i}(z_{j,i})$ are: 
% \footnote{Part of the derivation here is for computation convenience and does not strictly follow probabilistic properties. For example, calculation of $\rvv_{j,i;\land}$ assumes probabilistic independence between $\rvv_{j-i,i}$ and $\rvv_{j-1,i'}$, which might not hold because they might depend on same variables in $\rvv_{j-2, *}$, etc.}
\begin{align*}
    \rvv_{j,i;\text{true}} &= \bm{1} 
    &\rvv_{j,i;\text{chaining}} &= \left(\rvv_{j-1,i}^\top \sum_{r\in\gR} \alpha_{r,j,i}\mA_r\right)^\top
    \\
    \rvv_{j,i;\lnot} &= \bm{1}-\rvv_{j-1,i}
    &\rvv_{j,i;\text{copy}} &= \rvv_{j-1,i}
    \\
    \rvv_{j,i;\land} &= \rvv_{j-1,i} \odot \sum_{i'=1}^m \beta_{j,i,i'}^\land \rvv_{j-1,i'}
    &
    \rvv_{j,i;\lor} &= \bm{1} - (\bm{1}-\rvv_{j-1,i}) \odot (\bm{1}-\sum_{i'=1}^m \beta_{j,i,i'}^\lor \rvv_{j-1,i'})
\end{align*}
where $\odot$ denotes Hadamard product. Note that we pose normalization constraints so that $\alpha_{r,j,i}>0, ~\sum_r\alpha_{r,j,i}=1,~\beta_{j,i,i'}^*>0,~
\sum_{i'}\beta_{j,i,i'}^*=1$. These 6 types of scores are then gathered by a probability distribution $p_{j,i,*}$:
\[
\rvv_{j,i}=
p_{j,i,1}\rvv_{j,i;\text{true}}
+p_{j,i,2}\rvv_{j,i;\text{chaining}}
+p_{j,i,3}\rvv_{j,i;\lnot}
+p_{j,i,4}\rvv_{j,i;\text{copy}}
+p_{j,i,5}\rvv_{j,i;\land}
+p_{j,i,6}\rvv_{j,i;\lor}
\]
Thereby $\rvv_{j,i}$ represents the result of the probabilistic logical function $f^\Theta_{j,i}$ on all entities. $p,\alpha,\beta$ are all learnable parameters in $\Theta$. There are a total of $T+1$ columns of intermediate functions. Finally we use the last column of functions $f^\Theta_{T,i}$ as $L^\Theta_i$, and $\mL^\Theta(e)=(L_1^\Theta(e), \cdots, L_m^\Theta(e))$ is our logical entity representation \model{} on $e$.

Next we explain the computation of chain-like probabilistic logical rules, and how to further incorporate \model{}. In \cite{yang2017differentiable}, they model a probabilistic selection of logical predicates, so that the rules can be differentiably evaluated. Suppose for the chain-like rules in Equation~\ref{eq:chain_rule}, the predicate of $r_k$ is selected according to a distribution $a_{r,k}$. Then the probability that the clause body is true between each $x, y\in\gE$ can be given by 
\begin{equation}
    \prod_{k=1}^K\left(\sum_{r\in\gR} a_{r,k}\mA_{r}\right)
    \label{eq:chain_rule_evaluation}
\end{equation}

Now we want to also add a logical function constraint $L^\Theta_{i_k}$ from $\mL^\Theta$.
% We remember that $L^\Theta_{i_k}(z_k)$ can be represented as a $|\gE|$-dimensional vector when $z_k$ is iterated over $\gE$. 
% Also note that we can write $L^\Theta_{i_k}(z_k)={\mL^\Theta}^\top \rvi_k$ where $\rvi_k$ is an one-hot vector with only $i_k$ being 1, 
Denote $\mL^\Theta(\gE)$ as an $m\times|\gE|$ matrix by iterating $\mL^\Theta(e)$ over all $e\in\gE$. 
We can select $L^\Theta_{i_k}$ from $\mL^\Theta$ according to a probabilistic distribution $\boldsymbol{\rho_k}$ over $[1..m]$. Then the results of $L^\Theta_{i_k}(z_k)$ on $\gE$ can be written in vector form ${\mL^\Theta(\gE)}^\top \boldsymbol\rho_k$. Finally, the evaluation of the body in Equation~\ref{eq:extended_rule} can be written as
\begin{equation}
    \prod_{k=1}^{K}
    \left(
        \sum_{r\in\gR} a_{r,k}\mA_{r}
    \right)
    \text{diag}\left({\mL^\Theta}^\top \boldsymbol\rho_k\right)
    \label{eq:evalution}
\end{equation}
\input{tables/link_prediction}

This is the evaluation for a single logical rule. In practice we can have multiple rules to predict one target relation (e.g., in DRUM, there are up to 4), and there are multiple types of target relations in the dataset. So, we learn individual sets of parameters $a_{r,k}$ and $\boldsymbol\rho_k$ for different rules, but the parameter $\Theta$ for \model{} is shared across rules.




\subsection{Reasoning and Training}

In the task of knowledge graph completion, the model is given a set of queries $r(h,?)$ and required to find the entity $t\in\gE$ that satisfies relation $r(h,t)$. During reasoning and training, we denote $\rvh$ as the one-hot vector of entity $h$, and multiply it with Equation~\ref{eq:evalution} to calculate
\begin{equation*}
   \hat{\rvt}^\top = \rvh^\top\prod_{k=1}^{K}
    \left(
        \sum_{r\in\gR} a_{r,k}\mA_{r}
    \right)
    \text{diag}\left({\mL^\Theta}^\top \boldsymbol\rho_k\right)
\end{equation*}

This then can be calculated as a sequence of vector-matrix multiplications. The resulting vector is indicating which entity $t$ is satisfying the query $r(h,?)$. For training criterion, we use the cross entropy between the normalized prediction $\frac{\hat{\rvt}}{\|\hat{\rvt}\|_1}$ and ground-truth one-hot vector $\rvt$. The loss is differentiable with respect to all the parameters in our model, so we can apply gradient-based optimization methods such as Adam~\citep{kingma2014adam}. During evaluation, we use $\hat{\rvt}$ as scores and sort it to obtain a ranked entity list for calculating mean reciprocal rank (MRR), Hits, etc.

==> body/60_experiments.tex <==
\label{sec:experiments}

% \heng{\sout{unclear what baselines you are comparing to. Ideally it should be some method that does not use logical rule representation, and also do ablation test to show the impact of entity context}}

\input{tables/discovered_rules.tex}
\input{tables/logical_functions.tex}
\subsection{Knowledge Graph Completion}
\input{body/61_graph_completion.tex}

\input{figures/visualization.tex}
\subsection{Interpretability of LERP and logical rules}
\input{body/62_interpretability.tex}

\input{figures/hyperparameter}
\subsection{Model Analysis}
\input{body/63_hyperparameters.tex}

\input{tables/TransE_functions.tex}
% \subsection{Combining \model{} with Embedding Learning Models}
\subsection{Augmenting Embedding Learning Models with \model{}}
% \subsection{TransE + \model{}}
\input{body/64_TransE.tex}

% \subsection{Answering Logical Queries}

==> body/64_TransE.tex <==
\label{subsec:TransE} 

\model{} is designed to learn an interpretable logical representation for entities in graphs. One question then arises: can \model{} work together with other embedding-learning methods such as TransE~\citep{bordes2013translating}, to combine the logic structure in \model{} and strong fitting power of TransE?
Inspired by this idea, we design a hybrid model TransE+\model{}. We use the training framework and training criterion on TransE, but the entities' embeddings are now defined as $Embed'(e) = Embed(e)+R\boldsymbol{L^\Theta}(e)$. $Embed(e)$ is set as a 20-dimensional entity-specific embedding. We also set the width and depth of \model{} to be 8 and 2. $R$ is a $20\times8$ matrix to transform  \model{} to the embedding space. Besides the loss in original TransE framework, we add a regularization term $\eta \frac{\sum_e \|Embed(e)\|_2}{\sum_e \|R\boldsymbol{L^\Theta}(e)\|_2}$ to encourage \model{} to encode important information during optimization. We also introduce an advanced version TransE+\model{}+entropy by adding an extra entropy regularization term $\gamma H(\Theta)$ on \model{}'s weights. This term is added to loss and encourage \model{} to assign more weights to fewer logical rules. In experiments, we set $\eta=10$ and $\gamma=1$.

\input{figures/TransE_family.tex}
We evaluate the models on Family dataset and results are presented in Figure~\ref{fig:transe_family}. The vanilla TransE model tends to overfit the training set ($>$95\% training set accuracy) because Family dataset contains a limited number of training triplets. TransE+\model{} achieves higher test set performance. We hypothesize that \model{} provides logical regularization on the embedding $Embed'(e)$ and makes it more generalizable. After adding the entropy regularization term, the performance further improves. We attribute this to that the regulation encourages learning more explicit logical functions, which serves as a prior in embedding learning.

We also study the interpretability of the hybrid model. In Table~\ref{tab:TransE_functions} we list the logical functions that are learned by TransE+\model{}. There are 2 repetitions in logical functions which are removed. We also manage to identify the correlation between relations in TransE and logical functions. In TransE, each relationship has a vector $\vl$ to denote a translation in the embedding space. $\vl$ resides in the embedding space, and we want to find a vector $\vl'$ in \model{} space so that $R\vl'\approx \vl$. As $R$ is not square matrix, we use $R$'s Moore–Penrose inverse $R^+$ to project the translation vectors to $R^+\vl$. We then look for dimensions with highest values in $R^+ \vl$, and results are listed in the 2nd and 4nd columns in Table~\ref{tab:TransE_functions}. We can observe that these functions encode rich information. For example, relations like \textit{daughter} and \text{niece} are associated with $\exists z: niece(e,z)$ which suggests a female gender and lower rank in the family tree.

==> figures/TransE_family.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\centering
\includegraphics[width=0.5\textwidth]{figures/TransE_family.pdf}

% \vspace{-2mm}
\caption{Incorporating LERP representation improves TransE's performance on Family dataset.}
% \vspace{-2mm}
\label{fig:transe_family}
\end{wrapfigure}

==> figures/motivating_study.tex <==
\begin{wrapfigure}{r}{0.7\textwidth}
\centering
\includegraphics[width=0.7\textwidth]{figures/motivating_study_fig.pdf}

\vspace{-2mm}
\caption{Results in a motivating study on Family and Kinship dataset~\citep{kok2007statistical}.}

\label{fig:motivating_study}
\end{wrapfigure}

==> tables/TransE.tex <==
% \begin{figure}
% \begin{floatrow}
% \ffigbox{%
% }{%
% \centering
% \includegraphics[width=0.5\textwidth]{figures/TransE_family.pdf}

% \vspace{-2mm}
% \label{fig:transe_family}
% \caption{Incorporating LERP representation improves TransE's performance on Family dataset.}
% }
% % \capbtabbox{%
% \begin{table}
%   \begin{tabular}{cc} \hline
%   Author & Title \\ \hline
%   Knuth & The \TeX book \\
%   Lamport & \LaTeX \\ \hline
%   \end{tabular}
% % }{%
%   \caption{A table}%
% % }
% \end{table}
% \end{floatrow}
% \end{figure}


% \begin{table}
% \centering
% \setlength{\tabcolsep}{2mm}{

% \subfloat[Results of incorporating LERP into TransE framework.]{
% \begin{tabular}{lcccc}
% \toprule
% & \multicolumn{4}{c}{Family} \\
% & MRR & H@1 & H@3 & H@10 \\
% \midrule
% TransE & 0.263 & 0.089 & 0.353 & 0.625 \\
% + LERP & 0.300 & 0.102 & 0.408 & 0.700 \\
% + LERP + entropy & 0.355 & 0.162 & 0.474 & 0.728 \\
% \bottomrule
% \end{tabular}
% }
% \quad
% \subfloat[Prominent logical functions discovered by TransE framework with LERP representation.]{
% \begin{tabular}{cc}
% \toprule
% weight & logical function \\
% \midrule
% Aunt & $\not\exists z: uncle(e,z)$ \\
% Daughter & $\exists z: niece(e,z)$ \\
% Father & $\not\exists z: niece(e,z)$ \\
% Husband & $\not\exists z: niece(e,z)$ \\
% % Nephew & $\exists z_1,z_2: mother(z_1,e) \land niece(z_1,z_2)$ \\
% \bottomrule
% \end{tabular}
% }

% }
% \end{table}
